Passport: Enabling Accurate Country-Level Router Geolocation using Inaccurate Sources

When does Internet traffic cross international borders? This question has major geopolitical, legal and social implications and is surprisingly difficult to answer. A critical stumbling block is a dearth of tools that accurately map routers traversed by Internet traffic to the countries in which they are located. This paper presents Passport: a new approach for efficient, accurate country-level router geolocation and a system that implements it. Passport provides location predictions with limited active measurements, using machine learning to combine information from IP geolocation databases, router hostnames, whois records, and ping measurements. We show that Passport substantially outperforms existing techniques, and identify cases where paths traverse countries with implications for security, privacy, and performance.

==> countries-ground.tex <==
\begin{center}
%\begin{table}[]
%    \centering
%	\minipage{\columnwidth}
    \rowcolors{2}{gray!10}{white}
%    \caption{My caption}
    \bottomcaption{\textbf{Number of instances per country in entire ground truth dataset.} {\sl The complete list of countries (and independent territories) used by our \ensemble classifier to train, initially. 65\% of the countries have four or more instances in our initial training dataset. A visual representation of the top 20 countries is available in Figure \ref{fig:ground_truth_countries_stats}.}} 
    \begin{supertabular}{l | l}
        \textbf{Country}         & \textbf{Count} \\ \hline
        United States            & 2911  \\
        United Kingdom           & 1323  \\
        Germany                  & 923   \\
        France                   & 781   \\
        Netherlands              & 437   \\
        Australia                & 399   \\
        Russia                   & 367   \\
        Sweden                   & 335   \\
        Brazil                   & 314   \\
        South Africa             & 302   \\
        Canada                   & 218   \\
        Japan                    & 207   \\
        Italy                    & 190   \\
        Poland                   & 174   \\
        China                    & 215   \\
        Spain                    & 159   \\
        Austria                  & 155   \\
        Singapore                & 148   \\
        Ukraine                  & 145   \\
        Switzerland              & 144   \\
        Czech Republic           & 143   \\
        Norway                   & 105   \\
        India                    & 105   \\
        Finland                  & 102   \\
        Ireland                  & 89    \\
        Hungary                  & 89    \\
        Denmark                  & 79    \\
        New Zealand              & 74    \\
        Belgium                  & 73    \\
        Greece                   & 57    \\
        Turkey                   & 52    \\
        Romania                  & 46    \\
        Bulgaria                 & 46    \\
        Slovenia                 & 45    \\
        Kenya                    & 36    \\
        South Korea              & 36    \\
        Portugal                 & 35    \\
        Luxembourg               & 34    \\
        Slovakia                 & 32    \\
        Argentina                & 27    \\
        Indonesia                & 23    \\
        Israel                   & 21    \\
        Kazakhstan               & 21    \\
        Mexico                   & 20    \\
        Taiwan                   & 19    \\
        Lithuania                & 17    \\
        Estonia                  & 16    \\
        Uruguay                  & 16    \\
        Thailand                 & 15    \\
        Croatia                  & 13    \\
        Pakistan                 & 13    \\
        Qatar                    & 13    \\
        Bhutan                   & 12    \\
        Tanzania                 & 12    \\
        Malaysia                 & 11    \\
        Georgia                  & 11    \\
        Tajikistan               & 10    \\
        Madagascar               & 9     \\
        Uganda                   & 9     \\
        Iceland                  & 8     \\
        Latvia                   & 7     \\
        Namibia                  & 7     \\
        Iran                     & 7     \\
        Mozambique               & 7     \\
        Belarus                  & 7     \\
        Venezuela                & 6     \\
        Bangladesh               & 6     \\
        Botswana                 & 6     \\
        Chile                    & 6     \\
        United Arab Emirates     & 6     \\
        Kuwait                   & 6     \\
        Malawi                   & 5     \\
        Saudi Arabia             & 5     \\
        Zimbabwe                 & 5     \\
        Sudan                    & 5     \\
        Cyprus                   & 5     \\
        Serbia                   & 5     \\
        Vietnam                  & 5     \\
        Philippines              & 4     \\
        Gambia                   & 3     \\
        Morocco                  & 3     \\
        Armenia                  & 3     \\
        Ghana                    & 3     \\
        Honduras                 & 3     \\
        Costa Rica               & 3     \\
        Seychelles               & 3     \\
        Ecuador                  & 3     \\
        Faroe Islands            & 3     \\
        Maldives                 & 3     \\
        Sri Lanka                & 3     \\
        Bosnia                   & 3     \\
        Peru                     & 2     \\
        Senegal                  & 2     \\
        U.S. Virgin Islands      & 2     \\
        Moldova                  & 2     \\
        Nepal                    & 2     \\
        Northern Mariana Islands & 2     \\
        Azerbaijan               & 2     \\
        Egypt                    & 2     \\
        Zambia                   & 2     \\
        Djibouti                 & 2     \\
        Gibraltar                & 1     \\
        Paraguay                 & 1     \\
        Swaziland                & 1     \\
        Vanuatu                  & 1     \\
        Benin                    & 1     \\
        Guatemala                & 1     \\
        Kyrgyzstan               & 1     \\
        Nigeria                  & 1     \\
        Panama                   & 1     \\
        Phillipines              & 1     \\
        Reunion                  & 1     \\
        Saint Helena             & 1     \\
        Syria                    & 1     \\
        Albania                  & 1     \\
        Colombia                 & 1     \\
        Ivory Coast              & 1     \\
        Rwanda                   & 1     \\
        Bolivia                  & 1     \\
        Cuba                     & 1     \\ \hline
        \emph{Total}             & \emph{\numTrainSize} \\
    \end{supertabular}
	\vspace{\postfigspace}
	\label{tab:country_ground_truth_complete_list}
%\end{table}
\end{center}

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}

%\artbd{Note one line contains one sentence in this tex file. This is useful to track diffs between successive commits.}


